Measurement of the liquid argon energy response to nuclear and electronic recoils

A liquid argon time projection chamber, constructed for the Argon Response to Ionization and Scintillation (ARIS) experiment, has been exposed to the highly collimated and quasi-monoenergetic LICORNE neutron beam at the Institute de Physique Nuclaire Orsay in order to study the scintillation response to nuclear and electronic recoils. An array of liquid scintillator detectors, arranged around the apparatus, tag scattered neutrons and select nuclear recoil energies in the [7, 120] keV energy range. The relative scintillation efficiency of nuclear recoils was measured to high precision at null field, and the ion-electron recombination probability was extracted for a range of applied electric fields. Single Compton scattered electrons, produced by gammas emitted from the de-excitation of $^7$Li* in coincidence with the beam pulse, along with calibration gamma sources, are used to extract the recombination probability as a function of energy and electron drift field. The ARIS results have been compared with three recombination probability parameterizations (Thomas-Imel, Doke-Birks, and PARIS), allowing for the definition of a fully comprehensive model of the liquid argon response to nuclear and electronic recoils down to a few keV range. The constraints provided by ARIS to the liquid argon response at low energy allow the reduction of systematics affecting the sensitivity of dark matter search experiments based on liquid argon

==> Conclusions.tex <==
% !TEX root = aris_q_paper.tex
\section{Conclusions}

The scintillation yield of nuclear recoils relative to electronic recoils between $\sim$7~keV$_{nr}$ and $\sim$120~keV$_{nr}$ has been measured in LAr using a highly collimated and quasi-monoenergetic neutron source. This work presents the most precise measurement and lowest energy probe of \Leff, the nuclear recoil scintillation efficiency  in LAr. 

In addition, Compton scattered electrons induced by $\gamma$s from \Lim de-excitation, in coincidence  with the neutron beam, are used to measure the relative scintillation LY  as a function of energy and drift field along with $\gamma$s from calibration sources.  At null field, the LY  was measured to be constant within 1.6\% in the [40, 511]~keV$_{ee}$ range, the most stringent test of the linearity of the LAr response. Furthermore, no differences were observed in the light response   between single- and multi-scatter ER events. 

In presence of an electric field, three models (Thomas-Imel, Doke-Birks, and PARIS) were compared to the NR and ER data sets. The Thomas-Imel electron-ion recombination probability function, properly tuned on these data, provides a good description of the response to NRs at different fields, while PARIS is confirmed as a good model for ERs at the DarkSide-50 operation drift field of 200 V/cm.  The   Doke-Birks recombination probability models the response to ERs at different fields, but only above 40~keV$_{ee}$, in the upper range  of interest for dark matter searches. 

Finally, a comparison of the ionization signal between the tuned Thomas-Imel model and an independent NR data set at 6.7~keV$_{nr}$ suggests  that no extra quenching factors are required to predict  the number of ionization electrons.% with drift field in the range below 700~V/cm. 

In conclusion, this work provides a fully comprehensive model of the  LAr response in the range of interest for dark matter searches through measurement of the \Leff parameter as a function of NR energy, and by properly tuning the parametrization of the electron-ion recombination  probabilities for  ERs and NRs. 
 
%We have measured the scintillation yield of nuclear recoils relative to electron recoils between 6.99 keV and 119.4 keV in liquid argon.  This is both the highest precision and lowest recoil energy measurement of \Leff  to date.  This result is useful for calibration of dark matter search experiments such as DarkSide which utilize LAr as a detection medium.

%The Compton scattered electrons coincident with the neutron beam pulse are used to measure the relative light yield as a function of energy and electron-ion recombination probability of the LAr response to single-scatter electronic recoil events. 
%The LAr light yield as a function of ER energy is confirmed to be constant within 5\%, agreeing with previous published results and providing the first single-scatter data for this measurement. 
%This result is important in the construction and calibration of models which predict the behavior of LAr to recoiling electrons.
%The recombination probability of ER events
%	We also make the first direct measurement of the linearity  and recombination probability of the LAr scintillation response with respect to recoil energy using single Compton scatter events produced in coincidence with the neutron beam.  We make a confirmation of the linearity of the liquid argon light yield to within 4\%.  These results should be useful for making accurate calibrations of models which predict behavior of liquid argon, such as NEST.

%The behavior of the pulse shape discrimination parameter \FNine for ER and NR events was presented as a function of both recoil energy and electric field.  An interesting behavior is observed where NR and ER events show opposite trends in the migration of \FNine as a function of applied electric field.  Further exploration of the \FNine parameter with these data may reveal the source of this behavior.

%would be valuable to LAr dark matter direct detection experiments.

==> aris_q_frontpage.tex <==
% !TEX root = aris_q_paper.tex
\newcommand{\APC}{APC, Universit\'e Paris Diderot, CNRS/IN2P3, CEA/Irfu, Obs. de Paris, Sorbonne Paris Cit\'e, Paris 75205, France}
\newcommand{ \AQGSSI}{Gran Sasso Science Institute, L'Aquila AQ 67100, Italy}
\newcommand{\AQLNGS}{Laboratori Nazionali del Gran Sasso, Assergi AQ 67010, Italy}
\newcommand{\Houston}{Department of Physics, University of Houston, Houston, TX 77204, USA}
\newcommand{\IHEP}{Institute of High Energy Physics, Beijing 100049, China}
\newcommand{\LPNHE}{LPNHE Paris, Sorbonne Universit\'e, Universit\'e Paris Diderot, CNRS/IN2P3, Paris 75252, France}
\newcommand{\MIINFN}{Istituto Nazionale di Fisica Nucleare, Sezione di Milano, Milano 20133, Italy}
\newcommand{\NAINFN}{Istituto Nazionale di Fisica Nucleare, Sezione di Napoli, Napoli 80126, Italy}
\newcommand{\NAUni}{Department of Physics, Universit\`a degli Studi Federico II, Napoli 80126, Italy}
\newcommand{\Princeton}{Department of Physics, Princeton University, Princeton, NJ 08544, USA}
\newcommand{\Temple}{Department of Physics, Temple University, Philadelphia, PA 19122, USA}
\newcommand{\Davis}{Department of Physics, University of California, Davis, CA 95616, USA}
\newcommand{\UCAS}{School of Physics, University of Chinese Academy of Sciences, Beijing 100049, China}
\newcommand{\UCLA}{Department of Physics and Astronomy, University of California, Los Angeles, CA 90095, USA}
\newcommand{\IPNO}{Institut de Physique Nuclaire Orsay, F91406 Orsay, France}
\newcommand{\GSSI}{Gran Sasso Science Institute, L'Aquila 67100, Italy}


\author{P.~Agnes}\affiliation{\Houston}\affiliation{\APC}
\author{J.~Dawson}\affiliation{\APC}
\author{S.~De~Cecco}\affiliation{\LPNHE}
\author{A.~Fan}\affiliation{\UCLA}
\author{G.~Fiorillo}\affiliation{\NAUni}\affiliation{\NAINFN}
\author{D.~Franco}\affiliation{\APC}
\author{C.~Galbiati}\affiliation{\Princeton}
\author{C.~Giganti}\affiliation{\LPNHE}
\author{T.~N.~Johnson}\email{tesjohns@ucdavis.edu}\affiliation{\Davis}
\author{G.~Korga}\affiliation{\Houston}\affiliation{\AQLNGS}
\author{D.~Kryn}\affiliation{\APC}
\author{M.~Lebois}\affiliation{\IPNO}
\author{A.~Mandarano}\affiliation{\GSSI}\affiliation{\AQLNGS}
\author{C.~J.~Martoff}\affiliation{\Temple}
\author{A.~Navrer-Agasson~}\affiliation{\LPNHE}
\author{E.~Pantic}\affiliation{\Davis}
\author{L.~Qi}\affiliation{\IPNO}
\author{A.~Razeto}\affiliation{\AQLNGS}
\author{A.~L.~Renshaw}\affiliation{\Houston}
\author{Q.~Riffard}\email{riffard@apc.in2p3.fr}\affiliation{\APC}
\author{B.~Rossi}\affiliation{\NAINFN}
\author{C.~Savarese}\affiliation{\GSSI}\affiliation{\AQLNGS}
\author{B. Schlitzer}\affiliation{\Davis}
\author{Y.~Suvorov}\affiliation{\Houston}\affiliation{\AQLNGS}
\author{A.~Tonazzo}\affiliation{\APC}
\author{H.~Wang}\affiliation{\UCLA}
\author{Y.~Wang}\affiliation{\UCLA}
\author{A.~W.~Watson}\affiliation{\Temple}
\author{J.~N.~Wilson}\affiliation{\IPNO}

\collaboration{The ARIS Collaboration}\noaffiliation





==> introduction.tex <==
\section{Introduction}

The field of direct dark matter searches has experienced a significant expansion in the past decade, with a growing number of experiments striving to increase the sensitivity to signals from dark matter particles.
%with many new experiments coming on board and exploring new avenues to increase sensitivity to dark matter particles. All of them are trying to identify dark matter by detecting its possible interaction with ordinary matter in specialized, low-background detectors deployed in underground laboratories. 
Direct dark matter search experiments seek a possible interaction between dark matter and Standard Model matter in specialized, low-background detectors deployed in underground laboratories. 
The absence of an unambiguous observation of Weakly Interacting Massive Particle (WIMP) signals in recent years has pushed experiments to increase their sensitivity by simultaneously reducing the background, enlarging the active detector volume, and lowering the energy threshold of the searches. 

In this context, noble liquids are ideal candidates as target materials: they are relatively inexpensive, intrinsically more pure than other materials, and  scalable to masses in the multi-ton range. Further, they guarantee an excellent detector resolution through high ionization and scintillation photon yields. 

Dual-phase noble liquid time projection chamber (TPC) detectors are currently the most sensitive detectors in searches for multi-GeV mass WIMPs ~\cite{Aprile:2017tt,Akerib:2017kg,Tan:2016fv}. The detection mechanism relies on the delayed coincidence between scintillation and ionization signals generated by the passage of an interacting particle. 
The prompt scintillation light (S1 signal) is produced by the decay of excited dimers of noble atoms, which are formed after one atom is excited.  
Interactions also produce ionization electrons, drifted by an electric field toward a gaseous region, where they produce a delayed light pulse by electroluminescence (S2 signal).  
A fraction of free electrons, however, recombine with ions to form excited dimers which contribute to S1 and deplete the S2 signal.

With respect to other noble liquid targets, liquid argon (LAr) exhibits a powerful rejection of electronic recoil backgrounds ($>$10$^8$ discrimination power \cite{Amaudruz:2016qqa}) through the temporal pulse shape of the scintillation signal.  
The combination of this pulse-shape discrimination technique and the use of argon extracted from deep underground, highly depleted in cosmogenic isotopes~\cite{Agnes:2016fz}, makes liquid argon an ideal target for multi-ton detectors. 


The sensitivity of liquid argon detectors can be enhanced by constraining the parameters of the liquid argon response to interacting particles, such as the quenching of nuclear recoils and the electron-ion recombination effect. These parameters are difficult to constrain in large detectors with external sources, because of the passive materials which suppress interactions in the target.  Alternatively, the liquid argon response can be measured by auxiliary calibration experiments which exploit small-scale detector setups exposed to neutron and gamma beams.  These experiments, tailored specifically for measurements of the liquid argon response, are able to accurately explore the low energy ranges for nuclear and electronic recoils under controlled conditions.



The ARIS (Argon Response to Ionization and Scintillation) experiment is a fixed kinematics scattering experiment utilizing a LAr TPC aimed to investigate the response of LAr to nuclear and electronic recoils, with nuclear recoils measured down to $\sim$2~keVee (electron equivalent energy).
The ARIS TPC was exposed to the LICORNE pulsed neutron source at the ALTO facility in Orsay, France \cite{WILSON201431}.  The LICORNE source exploits the \Lipn inverse kinematic reaction, which guarantees a highly collimated and quasi-monoenergetic ($\sim$1.5~MeV) neutron beam, and at the same time, 
monoenergetic gammas from the 478~keV $^7$Li* de-excitation in coincidence with the beam pulse. Neutrons and gammas scattered in the TPC  are detected by an array of eight liquid scintillator detectors (labelled A0 to A7) which constrain the recoil energy in the TPC through the detector angle with respect to the TPC-beam axis. A picture of the setup is shown in figure~\ref{fig:aris_setup}.

\begin{figure}[t]
\includegraphics[width=0.99\columnwidth]{ARIS_setup3.pdf}
\caption{Picture of the ARIS setup in the LICORNE hall.}
\label{fig:aris_setup}
\end{figure}


In this work, we report on the precise measurement of the LAr scintillation efficiency for nuclear and electronic recoils at null field, and the dependence of the electron-ion recombination effect on the electric field.  



==> linearity.tex <==
% !TEX root = aris_q_paper.tex

%\section{Light yield linearity}
\section{Response to electron recoils at null field}
\label{sec:linearity}
%\blue{Editor: Quentin}


% 1) cite DEAP \cite{Amaudruz:2017ekt} and Lippincott  \cite{Lippincott:2010jb} for the linearity but explain this is done with gammas
Existing measurements  \cite{Lippincott:2010jb} suggest that the LAr response at null field to ERs is linear and hence not subjected to energy dependent quenching effects, unlike what has been observed in liquid xenon~\cite{Aprile:2006kx}.  Previous measurements of the linearity of the ER response in LAr have relied on multiple-scatter sources, such as the multi-step decay of \mKr and  $\gamma$ sources in the Compton-scattering dominated regime.  Direct measurements from single electronic recoils have not yet confirmed the linearity.

The eight single ER energies from Compton scattering of the mono-energetic $\gamma$ emitted by the \Lim de-excitation, tagged with the eight NDs, are ideal candles for this test.  
Data from the TPC is background subtracted as described in section~\ref{sec:selection}, and the resulting peak is fit with a Gaussian function. The LY  for Compton scatters tagged by NDs is evaluated  as a function of the  Compton electron energy determined with Monte Carlo simulation. 
The LY of each ND tagged dataset is found relative to the mean value of the set of eight measurements, and the relative LYs are fit with a first degree polynomial resulting in a maximum deviation from unity of 5\%   in the [41.5, 300]~keV range.
The value of this deviation includes the statistical error from the fit. 
%The so-obtained relative LYs, with respect to their mean value, are fit with a first degree polynomial resulting in a maximum deviation from unity of 5\%   in the [41.5, 300]~keV range, including the statistical error from the fit. 

The LY values independently extracted from the full absorption $\gamma$ peaks, shown in figure~\ref{fig_calib_ly_compton},  from  \am (59.5~keV), \ba (81 and 356~keV), and \Na (511~keV), are fully compatible with the average LY derived from single Compton electrons. This is expected for the full absorption peaks of 59.5 and 81~keV $\gamma$s as they are dominated by the photoelectric effect. The 356 and 511~keV $\gamma$ interactions,  instead, are dominated by Compton scattering,  producing multiple lower energy electrons.
If they were subjected to a quenching stronger at low energies (as it is the case, for example, for organic liquid scintillator), the light yield derived from multiple scatter $\gamma$s should differ from the one derived from single scatter events.
%A quenching effect, like the one observed in organic liquid scintillator, which is stronger at low energy, would induce a difference between single scatter events and $\gamma$s in the Compton regime. amplify the effect The total quenching effect for $\gamma$s in the Compton regime would then be amplified with respect to single scatter events. 
 
Fitting simultaneously the \am, \ba, \Na, and Compton electrons, the LY in the  [41.5, 511]~keV range is constant within 1.6\%, as shown in figure~\ref{fig_calib_ly_compton}. This result confirms the linearity of the LAr scintillation response at null field also observed by Lippincott \textit{et al.}~\cite{Lippincott:2010jb}  at 3\%, using multiple scatter sources in the [41.5, 662]~keV range.  This result suggests    that, at null field,  ERs are not subjected to non-linear quenching effects and that   calibrations of LAr detectors can be  performed either with single or multiple scatter ER sources without introducing any bias. 





 
\begin{figure}[t]
\includegraphics[width=\columnwidth]{linearity_compton.pdf}
\caption{
The relative  LY,  with respect to the mean,  as a function of the Compton electron energy from \Lim de-excitation, and from \am (59.5~keV), \ba (81 and 356~keV), and \Na (511~keV) $\gamma$ sources. The vertical error bars represent the statistical errors on LY while the horizantal error bars represent the uncertainties on the energy. All the data points are fit with a first degree polynomial (blues line)  to test for deviations from unity. The dashed red lines correspond to $\pm$1.6\% band and contain the fitted polynomial, including 1$\sigma$ error (blue band), in the [41.5, 511]~keV range.    }
\label{fig_calib_ly_compton}
\end{figure}






==> monitor.tex <==
% !TEX root = aris_q_paper.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Neutron beam and detectors calibration}
%\label{sec:monitor}
%\blue{Editor: Quentin}
%In this section we will describe the measurement of the neutron beam kinematics, the characterization of the TPC response, including the estimation of the LAr photoelectron yield (light-yield, LY) and of the trigger efficiency, and  the time resolution %obtained in the Time Of Flight (ToF) measurements between beam and TPC and beam and neutron detectors. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Neutron beam kinematics}
%\subsection{Neutron beam kinematics}
\label{sec:BeamKinematics}

The LICORNE neutron beam exploits the inverse kinematic reaction resulting from accelerated \Li incident on a gaseous hydrogen target.  The kinematics of the neutrons emitted from the \Lipn reaction highly depends on the energy of the \Li at the reaction site.  The \Li beam is initially accelerated to 14.63~MeV, and a fraction of its energy is lost as it crosses the tantalum foil containing the hydrogen target.  The exact thickness of the foil, and therefore the final \Li energy, is not well known.  A dedicated measurement was performed to determine the \Li energy at the reaction site, and therefore the kinematic profile of the neutron beam.  One ND was placed at a distance of 3~m from the source at angles varying between 0 and 15$^\circ$.  The relative neutron beam intensity with respect to the intensity at 0$^\circ$ was measured at each angle.  The resulting profile was compared with the results of a GEANT4 simulation developed to predict neutron spectra as a function of \Li energy \cite{Lebois:2014il}, which assumes different thicknesses of the tantalum foil. 

%Neutrons are emitted  from the LICORNE source via the $^7$Li(p,n)$^7$Be reaction and the neutron kinematics entirely depends on the \Li energy before the reaction.  Although \Li is accelerated at 14.63~MeV, a fraction of its energy is lost in the  tantalum foil, used to contain the gaseous Hydrogen target. Since the foil thickness is unknown,  the  \Li energy at the entrance of the gaseous target, and hence the neutron kinematics, was determined with a dedicated measurement. One ND was placed at a distance of 3~m from the source at different angles, varying between 0 and 15$^\circ$. The relative neutron beam intensity, with respect to the one at 0$^\circ$,  measured at each angle was compared with  GEANT4 simulations \red{reference?}, assuming different thicknesses of the tantalum foil. 

The best fit of the  beam profile was obtained for a foil thickness of $2.06 \pm 0.08\,\mathrm{\mu m}$, corresponding to a mean \Li energy in the hydrogen target of $13.13 ^{+0.02}_{-0.01}\,\mathrm{MeV}$. 
The corresponding kinematic profile of the neutron beam, in neutron energy vs. angle with respect to the \Li beam axis, is shown in figure~\ref{fig_calib_kine_bestfit}. 
The TPC, located 1 m from the neutron source, is exposed to $<$2$^\circ$ of the neutron cone. 
The mean neutron energy in this region is 1.45~MeV with an RMS of 85~keV.

\begin{figure}
\includegraphics[width=\columnwidth]{monitor_kinematics_bestfit.pdf}
\caption{Neutron kinematic profile for a \Li energy of  13.13~MeV incident on the hydrogen target, determined from Monte Carlo simulations. The red box defines the geometrical acceptance of the TPC. } %Best fit of the kinematics: $E_{Li} = 13.13\,\mathrm{MeV}$ after $2.06\,\mathrm{\mu m}$ Ta foil. }
\label{fig_calib_kine_bestfit}
\end{figure}

In addition to neutrons, LICORNE isotropically emits a source of 478 keV $\gamma$s in the center of mass frame from either  the \Be decay or by the de-excitation of \Lim,  produced when \Li crosses the tantalum foil. 
The decay of \Be, with a half-life of $\sim$53 days, constitutes a source of constant accidental background within the beam pulse.
%The first represents a constant source of accidental background, given the $\sim$53 days of half life of \Be, while  
The \Lim $\gamma$s are emitted in coincidence with the beam pulse, and when detected in coincidence between the beam pulse, TPC, and a ND, provide an excellent source of single Compton electrons for investigating the LAr response to ERs. 
%\Lim $\gamma$s, detected in triple coincidence between the beam pulse, the TPC, and NDs, provide an excellent sample of single Compton electrons for investigating  LAr response to ERs.  
The \Lim $\gamma$s are subjected to a relativistic boost due to the motion of the \Lim nuclei, which increases their energy up to 6\% for a \Li energy of 14.63~MeV.  Since the \Lim energy at which  $\gamma$s are emitted can vary because of the energy loss in the source materials, a mean boost of  3\% and,  conservatively, a $\sigma$ of 3\% are assumed, resulting in  a $\gamma$ energy of 492$\pm$15~keV. 




% from \Lim de-excitation.  %of there are 478 keV $\gamma$s coming from the \Lim de-excitation.
%The \Lim can  be produced either from \Be decay or directly from the excitation of \Li crossing the source materials.  $\gamma$s from the decay of \Be,  ($\tau$$\sim$52 day), represent a constant source of accidental background, while \Lim produced by the de-excitation of \Li de-excites immediately producing $\gamma$s that are correlated with the beam and that will be used for TOF calibration and as a source of single-scatter ER in the TPCs.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Detector calibration}
%\subsection{TPC light yield and trigger efficiency}
\label{sec_calibration}


The TPC response to scintillation light was calibrated throughout the data taking period with  \am\ and \ba $\gamma$-sources placed on the outside surface of the dewar.  Dominant $\gamma$-lines able to cross the dewar walls and reach the active LAr mass are  59.5~keV from  \am  and  81.0~keV to 383.8~keV from \ba. 

\begin{figure}[!t]
\includegraphics[width=\columnwidth]{monitor_tba.pdf}
\caption{Relative light collection efficiency as function of the TBA. Larger values of TBA correspond to recoils closer to the bottom of the TPC.}
\label{fig:TBA}
\end{figure}

\begin{figure}[!htpb]
\includegraphics[width=\columnwidth]{monitor_ly_am.pdf}
\includegraphics[width=\columnwidth]{monitor_ly_ba.pdf}
\caption{\am (top) and \ba (bottom) spectra from source calibration of the TPC light-yield at 0~V/cm with an overlay of the best fit spectra. The $\chi^2/n.d.f$ is 20.7/29 for \am and 190.7/189 for \ba. The vertical dashed line represents the low threshold for the fit interval.}
\label{fig_calib_ly}
\end{figure}

The energy deposits of the $\gamma$s in the LAr active target are simulated with a Geant4-based Monte Carlo. Its output is converted to the S1 observable by convolving energy deposits in the LAr with a response function. The response function is generated with a toy Monte Carlo approach, taking into account  the light yield (LY),  Poisson fluctuations in the photon statistics, the non-uniformity of  the light collection along the vertical axis, and the PMT response. The last is measured by fitting 
the single photoelectron distribution obtained with a pulsed LED light fed to the TPC through an optical fiber.
%the single electron distribution obtained with an LED light fed to 
The single photoelectron distribution was monitored throughout the data taking period.
The topological uniformity in light collection is measured by looking at the TBA (top/bottom asymmetry)  observable, defined as the ratio between the light collected by the bottom PMT with respect to the total.  The light collection is expected to be larger at the bottom because the 3-inch PMT provides a larger  optical coverage and   quantum efficiency with respect to the 1-inch PMT array at the top. %In figure~\ref{fig:TBA}, the light response is shown as function of the vertical position, measured with the mean S1 of the fitted \am $\gamma$ peaks.  It is the ratio of light collected at different subranges of TBA with respect to a TBA=0.6, where the maximum number of events is collected for the source position used.
The $\gamma$s from the \am source are used to evaluate the dependence of the light collection  on the TBA.
In figure~\ref{fig:TBA}, the mean S1 of the \am $\gamma$ peaks observed in different subranges of TBA is shown with respect to S1 for TBA=0.6. TBA=0.6 corresponds to the mean value of the TBA for events induced by a source placed at the center of the TPC.
%The light response is determined as the ratio of the mean S1 of the fitted \am $\gamma$ peaks, in different  subranges of TBA, with respect to TBA=0.6 where the maximum of events are collected for a height of the source at the TPC center.  




The \am and \ba data are then fit with the simulated distributions with the LY as the only free parameter.  The \am and \ba spectra and best fit Monte Carlo distributions are shown in figure~\ref{fig_calib_ly}.  A $\chi^2/ndf\sim1$ is achieved for both sources, showing that  data and Monte Carlo are in excellent agreement. 
A slow 1.8\% decrease in the LY over the period of data taking, likely due to variations in the LAr purity,  was observed with daily calibrations with the $\gamma$ sources, resulting in the dominant systematic error on the LY measurement.
%The uncertainty on the LY is dominated by the systematic error due to LY decreasing of 1.8\%  observed during the data taking  with daily calibrations with $\gamma$ sources. 
The best-fit is obtained for LY~=~6.35$\pm$0.05~pe/keV with the uncertainty including the systematic error on the LY stability.
The response map obtained for the average LY is shown in figure~\ref{fig_response_map}.

\begin{figure}[!htbp]
\includegraphics[width=\columnwidth]{fit_response_map.pdf}
\caption{The TPC optical response as a function of visible energy defined from the toy Monte Carlo approach described in the text.}
\label{fig_response_map}
\end{figure}



The trigger efficiency is derived with a dedicated measurement with a \Na source placed on the external wall of the dewar.  \Na emits a positron, resulting in two back-to-back 0.511~MeV $\gamma$s, simultaneous with an isotropic 1.27~MeV $\gamma$. Two BaF$_2$ detectors were  placed at a distance of $\sim2$~cm from the source: one on the TPC--\Na source axis in order to detect one of the two 0.511~MeV $\gamma$s from the positron annihilation, and the second  rotated by about 45 degrees with respect to the same axis to detect the isotropic 1.27~MeV $\gamma$. 
%This configuration constrains the direction of the second 0.511~MeV $\gamma$ toward the TPC center 
This trigger configuration provides selection of events where one 0.511~MeV $\gamma$ is directed toward the TPC center 
when both BaF$_2$ detectors are triggered.  In this case, the TPC event and  the TPC trigger status (two or more PMTs fire within 100 ns) are recorded along with the light  collected in the two BaF$_2$ detectors. 
Offline  cuts on the BaF$_2$ signals optimize the selection of  0.511~MeV $\gamma$-rays directed toward the TPC center, inducing a  Compton electron spectrum ensuring a trigger efficiency scan over the entire energy range of interest.  A dependence of the trigger efficiency on the TBA is expected due to the asymmetry in the photosensor setup on the top and bottom of the TPC and the trigger condition.  


The trigger efficiency is measured as a function of the signal in the first 100 ns (S1$_{100}$), the same gate as the one used for the trigger. Monte Carlo simulation have demonstrated that ER and NR have the same trigger efficiency with respect to this variable.
The fraction of reconstructed events with a positive trigger status as a function of S1$_{100}$ is evaluated for  three regions of TBA, approaching 1 in the entire detector for S1$_{100}$ $>$6, as shown in figure \ref{fig_trigg_eff}. Beam data are corrected on an event-by-event basis by evaluating the corresponding S1$_{100}$ value.
% as shown in figure \ref{fig_A0_trigger} for NR sample selected by A0 with the lowest mean energy (7.1~keV$_{nr}$), and where the impact of the trigger efficiency is expected to be maximal. 
Figure \ref{fig_A0_trigger} shows the comparison of corrected and un-corrected NR spectra selected by coincidence with the A0 detector (7.1~keV$_{nr}$), where the impact of the trigger efficiency is maximal. 


\begin{figure}[t]
\includegraphics[width=\columnwidth]{monitor_trigger_efficiency_inset.pdf}
\caption{ The trigger efficiency, as a function of S1$_{100}$, measured with the $^{22}$Na source for three regions of TBA.   The  plateau at  high energies does not reach unity due to the inhibition time of 10 ms introduced after each trigger. Dark noise prevents the efficiency from reaching zero at  very low values of S1$_{100}$. }
\label{fig_trigg_eff}
\end{figure}

\begin{figure}[t]
\includegraphics[width=\columnwidth]{eff_comparison_A0.pdf}
\caption{The effect of the trigger efficiency correction on the NR energy spectrum for events selected by coincidence with A0, resulting in a mean NR energy of 7.1~keV$_{nr}$.  The impact of the trigger efficiency is maximal for this data point. }
\label{fig_A0_trigger}
\end{figure}

The TPC saturation has been investigated with the \Na source by comparing S1 with S1$_{late}$, the integral of the signal starting after the first 90~ns. This integral range is not affected by saturation since it is dominated by the slow component of the scintillation emission with a characteristic time of $\sim$1.6~$\mu$s. A deviation from the linearity between S1 and S1$_{late}$ is observed from S1=4000~pe, corresponding to more than 600~keV$_{ee}$. A similar study has been performed on the spectrum of NRs selected in the double coincidence trigger mode.  The prompt scintillation component in NRs is larger than for ERs, so the effect of saturation is expected at lower S1. Up to 400~pe, corresponding to the maximum energy of NRs induced by 1.45~MeV neutrons, no deviations from linearity were observed between S1 and S1$_{late}$.


A clock misalignment was occasionally observed on a run-by-run basis between the CAEN boards. To synchronize them,  a time calibration for each run was performed using the \Lim $\gamma$ signal from the triple coincidence trigger data. 
%The  $\gamma$ time-of-flight (TOF) between the beam pulse and both the TPC and the NDs, which are canceled by the synchronization, are accounted for in the data reconstruction.  
The TOF between the beam pulse and the TPC (\TPCtof) and the beam pulse and the NDs  (\NDtof) is shown in figure \ref{fig_tof_mc-data}, compared with  Monte Carlo simulations of neutrons for the A3 ND.  The time resolutions of the two TOFs are measured with  \Lim $\gamma$s to be 1.8 ns for the \TPCtof, and in the 2--3~ns range for the eight \NDtof and are included in the simulation. 
The excellent agreement in both TOF distributions is an indirect confirmation of the neutron kinematic profile assumed in the Monte Carlo.


\begin{figure}[t]
%\includegraphics[width=\columnwidth]{tof.pdf}
\includegraphics[width=\columnwidth]{mc_comparison_tof_beam_new.pdf}
\caption{Data and Monte Carlo comparisons of the \TPCtof (top) and  \NDtof (bottom) distributions for the A3 detector. The peak at 0~ns corresponds to the \Lim $\gamma$ that are not simulated in the MC. %The flat background in both of the simulation samples is produced  with  a toy Monte Carlo tuned on the data.
}
\label{fig_tof_mc-data}
\end{figure}

 


==> quenching.tex <==
% !TEX root = aris_q_paper.tex

\section{Response to nuclear recoils at null field}
\label{sec:quenching}
%\blue{Editor: Tessa}



The scintillation efficiency for nuclear recoils, $\mathcal{L}_{eff}$, is defined in this work with respect to the response of LAr to the 59.5~keV $\gamma$ from \am at null field. 
The comparison with other $\mathcal{L}_{eff}$ measurements~\cite{Gastler:2010sc,Cao:2015ks,Creus:2015fqa} using different reference sources (e.g. $^{57}$Co and \mKr) is guaranteed by the linearity of the ER response demonstrated in the previous section.  

S1 distributions of NR data samples, selected with a coincidence signal from each ND as described in section~\ref{sec:selection}, are independently fit with a probability density function derived from the  Monte Carlo.  The only free parameters in the fit are the normalization factor and \Leff, which acts as a scaling factor of the light yield. %\Leff is assumed to be constant for each data sample.  
Results from each fit are shown in figure~\ref{fig_fit_res_part2}.

\begin{centering}
\begin{figure*}[!ht]
\begin{minipage}{\textwidth}
	\includegraphics[width=2.80in]{quenching_ch0.pdf}
	\includegraphics[width=2.80in]{quenching_ch1.pdf}
	\includegraphics[width=2.80in]{quenching_ch2.pdf}
	\includegraphics[width=2.80in]{quenching_ch3.pdf}
	\includegraphics[width=2.80in]{quenching_ch4.pdf}
	\includegraphics[width=2.80in]{quenching_ch5.pdf}
	\includegraphics[width=2.80in]{quenching_ch6.pdf}
	\includegraphics[width=2.80in]{quenching_ch7.pdf}
	\caption{Nuclear recoil data taken with zero electric field, fitted with the Monte Carlo-derived probability density functions for events in coincidence with the A0-7 detectors (red lines).  The vertical dashed lines indicate the fitting range for each spectrum.}
	\label{fig_fit_res_part2}
\end{minipage}
\end{figure*}
\end{centering}


The sources of systematic error affecting this measurement are listed in table~\ref{tab_sys}. The dominant contributions to the uncertainty on \Leff are the uncertainties on the LY and on the ND positions. The first is evaluated with an analytical propagation of the error on the LY, while the second relies on Monte Carlo simulations where the ND positions were varied according to the uncertainty from the survey in the direction that maximizes the NR energy spread. The survey was done by measuring the distance of each ND from several reference points along the beam direction. An \textit{a posteriori} cross-check was done by overlaying several photographs of the entire setup with the rendering of the geometry in the Monte Carlo using the BLENDER software~\cite{BLENDER}. The TPC, the source position, and the ND support structures were used as reference anchors in the comparison. All ND positions were confirmed within a maximum shift of 4~cm with the exception of A2, which required a shift of (-6,+7,+13)~cm with respect to the survey position\footnote{x is the beam-TPC direction, z is the vertical coordinate, and y is orthogonal to the xz--plane.}. 
%The uncertainty on the A2 ND position is conservatively assumed of the same size of the shift corresponding to an uncertainty of 5.6\% on the NR energy. 
The size of the shift is conservatively assumed to be the uncertainty on the A2 position and, when propagated to the NR energy, results in an uncertainty of 5.5\%.
The uncertainty on the NR energy for coincidences with the other NDs ranges from 0.8\% to 2.5\%.   

Other subdominant sources of systematic error relating to the setup geometry and materials are the uncertainties on the \Li energy, with its determination described in section \ref{sec:BeamKinematics}, and the TPC position, known within 1~cm. Their impact on \Leff, quoted in table~\ref{tab_sys}, was evaluated with Monte Carlo simulations. Systematic effects associated with the analysis procedure, such as the trigger efficiency correction, the TOF cuts, histogram binning, energy range of the fit, and background subtractions were investigated by varying the associated parameters. Only the uncertainties on the trigger efficiency and the TOF selection induce a non--negligible systematic error on \Leff and are quoted in table~\ref{tab_sys}. 

\begin{figure*}
\includegraphics[width=0.7\textwidth]{results_quenching.pdf}
\caption{\Leff dependence on NR energy as measured by this work and compared with other data sets~\cite{Cao:2015ks, Gastler:2010sc, Creus:2015fqa} and models~\cite{Lindhard:1963,Mei:2008ca}.}
\label{fig_quenching}
\end{figure*}


\begin{table*}
  \centering
  \begin{tabular}{lC{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}}
    \hline
    \hline
    NR energy [keV] & 7.1 & 13.7 & 17.8 & 21.7 & 40.5 & 65.4 & 98.1 & 117.8\\ 
    \hline
    \Leff & 0.243 & 0.258 & 0.253 & 0.269 & 0.286 & 0.304 & 0.332 & 0.349    \\ 
    \hline
    Light-yield  & 0.002 & 0.002 & 0.002 & 0.002 & 0.002 & 0.002 & 0.003 & 0.003    \\ 
    Beam kinematic  & 0.001 & 0.002 & $o(10^{-3})$ & $o(10^{-3})$ & $o(10^{-3})$ & $o(10^{-3})$ & $o(10^{-3})$ & $o(10^{-3})$    \\ 
    A0--A7 position  & 0.006 & 0.005 & 0.014& 0.005 & 0.004 & 0.004 & 0.003 & 0.003    \\ 
    TPC position  & $o(10^{-3})$  & $o(10^{-3})$  & $o(10^{-3})$  & $o(10^{-3})$  & $o(10^{-3})$  & $o(10^{-3})$  & $o(10^{-3})$  & $o(10^{-3})$     \\ 
    A0--A7 TOF  & $o(10^{-3})$   & $o(10^{-3})$   & 0.001 & 0.001 & $o(10^{-3})$   & 0.002 & 0.001 & 0.001    \\ 
    TPC TOF  & 0.002 & 0.001 & 0.001 & 0.001 & 0.002 & 0.002 & 0.002 & 0.002    \\ 
    Trigger efficiency  & $o(10^{-3})$  & $o(10^{-3})$  & $o(10^{-3})$   & $o(10^{-3})$   & $o(10^{-3})$   & $o(10^{-3})$   & $o(10^{-3})$   & $o(10^{-3})$      \\ 
    \hline
    Total Syst. & 0.007 & 0.006  & 0.014  & 0.006  &  0.005 &  0.005 & 0.005  &   0.005    \\ 
    \hline
    Stat. & 0.005 & 0.004 & 0.003 & 0.002 & 0.003 & 0.006 & 0.004 & 0.002    \\ 
    \hline
    Combined & 0.009 & 0.007 & 0.015 & 0.006 & 0.006 & 0.008 & 0.006 & 0.005    \\ 
    \hline
    Combined relative [\%] & 3.8 & 2.7 & 5.8 & 2.3 & 2.1 & 2.6 & 1.8 & 1.5    \\ 
    \hline
    \hline
  \end{tabular}
  \caption{Measured \Leff for NR events coincident with each ND with the different sources of systematic uncertainties and the statistical uncertainty from the fit quoted.}
  \label{tab_sys}
\end{table*}

%\begin{table*}
%  \centering
%  \begin{tabular}{lC{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}}
%    \hline
%    NR energy [keV] & 7.14 & 13.72 & 17.78 & 21.69 & 40.45 & 65.37 & 98.14 & 117.78\\ 
%    \hline
%    $\mathcal{L}_{eff}$ & 0.24302 & 0.25843 & 0.25250 & 0.26851 & 0.28599 & 0.30423 & 0.33158 & 0.34895    \\ 
%    \hline
%    Stat. & 0.00544 & 0.00372 & 0.00274 & 0.00224 & 0.00340 & 0.00611 & 0.00375 & 0.00190    \\ 
%    \hline
%    Light-yield  & 0.00191 & 0.00203 & 0.00199 & 0.00211 & 0.00225 & 0.00240 & 0.00261 & 0.00275    \\ 
%    Beam kinematic  & 0.00133 & 0.00175 & 0.00004 & 0.00057 & 0.00070 & 0.00027 & 0.00053 & 0.00049    \\ 
%    A0--A7 position  & 0.00679 & 0.00507 & 0.01420 & 0.00507 & 0.00407 & 0.00366 & 0.00329 & 0.00287    \\ 
%    TPC position  & 0.00038 & 0.00021 & 0.00047 & 0.00025 & 0.00040 & 0.00052 & 0.00047 & 0.00048    \\ 
%    A0--A7 TOF cut  & 0.0  & 0.0  & 0.00102 & 0.00075 & 0.0  & 0.00153 & 0.00057 & 0.00100    \\ 
%    TPC TOF cut  & 0.00171 & 0.00146 & 0.00132 & 0.00138 & 0.00156 & 0.00163 & 0.00221 & 0.00238    \\ 
%    Trig. Eff  & 0.00021 & 0.00005 & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0     \\ 
%    \hline
%    Combined & 0.00918 & 0.00700 & 0.01470 & 0.00616 & 0.00602 & 0.00786 & 0.00611 & 0.00515    \\ 
%    \hline
%    Combined relative [\%] & 3.78 & 2.71 & 5.82 & 2.30 & 2.11 & 2.58 & 1.84 & 1.48    \\ 
%    \hline
%  \end{tabular}
%  \caption{Uncertainties as resulting from the fit (statistical) and from the different systematic sources affecting the \Leff measurement.}
%  \label{tab_sys}
%\end{table*}

This work provides the most precise determination of the \Leff dependence on the NR energy in LAr, as shown in figure~\ref{fig_quenching}, where it is compared with previous measurements~\cite{Cao:2015ks, Gastler:2010sc, Creus:2015fqa} and with existing models of quenching in LAr.  

The Lindhard theory~\cite{Lindhard:1963} predicts a quenching factor of
\begin{equation}
L_{eff}^{L}= \frac{kg(\epsilon)}{1 +  kg(\epsilon)},
\label{eq:lindhard} 
\end{equation} 
where \mbox{$\epsilon=11.5\, E_{NR}  Z^{-7/3}$}, \mbox{$k = 0.133\, Z^{2/3}\, A^{-1/2}$}, and \mbox{$g(\epsilon) = 3 \epsilon ^{0.15} + 0.7 \epsilon ^{0.6} + \epsilon$}, with $E_{NR}$ in keV and Z,A as the atomic and mass numbers.
The Mei model~\cite{Mei:2008ca} modifies the Lindhard expression by exploiting the Birks saturation law, 
\begin{equation}
L_{eff}^{M}= L_{eff}^{L} \times \frac{1}{1 + k_B \frac{dE}{dx}},
\label{eq:mei} 
\end{equation} 
where $k_B$ = 7.4$\times$10$^{-4}$ MeV$^{-1}$ g cm$^{-2}$.  Figure \ref{fig_quenching} shows that these models do not accurately represent the data.

Even if the values of $k$ or $k_B$ in the Lindhard or Mei models are left free and allowed to float in a fit, the NR data are still not accurately represented, with the Lindhard model disfavored at  $>$5$\sigma$ and the Mei model disfavored at 2$\sigma$.  However, the Mei model, modified by adding a quadratic term, 
\begin{equation}
L_{eff}^{M*}= L_{eff}^{L} \times \frac{1}{1 + k_B \frac{dE}{dx}+ k^{*}_B (\frac{dE}{dx})^2 },
\label{eq:mei2} 
\end{equation}
as in the extended version of the Birks'  formula for organic scintillators \cite{SMITH1968157}, is compatible with the data with a p-value of 0.79 using the best fit parameters of \mbox{$k_B$ = (5.2$\pm$0.6)$\times$10$^{-4}$ MeV$^{-1}$ g cm$^{-2}$} and \mbox{$k^{*}_B$ = (-2.0$\pm$0.7)$\times$10$^{-7}$ MeV$^{-2}$ g$^2$ cm$^{-4}$}.  This result is in agreement with the best fit of the modified Mei model to DarkSide-50 data which yields a value of \mbox{$k_B$ = (4.66$^{+0.86}_{-0.94}$)$\times$10$^{-4}$ MeV$^{-1}$ g cm$^{-2}$}~\cite{Agnes:2017grb}.  The three fitted models are shown with the ARIS data in figure~\ref{fig_quenching_models}.



%In the $\sim$[20, 60]~keV$_{nr}$ region the data sets are in good agreement, while discrepancies are observed outside of this range. At low energies, ARIS provides a \Leff measurement down to $\sim$7~keV$_{nr}$, the lowest NR energy  among the data sets. 




%Up to 60~keV$_{nr}$, ARIS data are in excellent agreement with the PARIS model, while at higher energies a larger \Leff is observed. In the same range there is a tension with the MicroCLEAN data that are in good agreement with the Mei model.

\begin{figure}
\includegraphics[width=\columnwidth]{quenching_models.pdf}
\caption{\Leff values measured by this work fit with Lindhard, Mei, and modified Mei models as described by equations \ref{eq:lindhard}, \ref{eq:mei}, and \ref{eq:mei2} in the text.}
\label{fig_quenching_models}
\end{figure}



%\begin{figure}
%\includegraphics[width=\columnwidth]{recombination_NR_field.pdf}
%\caption{Field induced quenching of S1 for \NRs\ for different drift fields. The systematic uncertainties are included in the error bars.  The inset shows the same data with the x-axis represented in a log-scale.}
%\label{fig:recombination_NR_field}
%\end{figure}


==> recombination.tex <==
% !TEX root = aris_q_paper.tex

\section{S1 response versus electric field}
%\blue{Editor: Paolo}


%\cmt{ Describe method (selection already described), discuss alpha for ER and NR} 
%blue{PA: Only a preliminary draft. the content (a review of the PARIS model in particular) depends on the content of the previous sections.} 
In addition to the null field data set, data were acquired  at 50, 100, 200,  and 500 V/cm drift fields in triple coincidence mode.  The presence of an electric field in the active volume increases the probability  that ionization electrons   escape the electron-ion cloud, reducing the recombination effect. 

Any energy deposit  in LAr   produces an average number of quanta ($N_q$), either  excitons or ion-electron pairs, corresponding to   

\begin{equation}
N_q =  N_i + N_{ex} =  \mathcal{L}_{eff} \times { E_{dep} \over  W } .
\end{equation}

where $W$=19.5~eV \cite{Doke:1988kw} is the effective work function,  $N_{ex}$  and    $N_{i}$  the numbers of excitons and ions, respectively, and  where $\mathcal{L}_{eff}$ is assumed to be 1 for \ERs. S1 can be expressed as function of  $\alpha$,  the   $N_{ex}$/$N_{i}$ ratio: 

\begin{equation}
S1    = \epsilon_1~(\alpha  + R) \times N_{i}
\label{eq:s1reco}
\end{equation}
where $\epsilon_1$ is the light collection efficiency of the detector, and $R$ the electron-ion recombination probability. The value of $\alpha$ is equal to 0.21  for ERs,  and to 1 for NRs~\cite{Doke:1988kw}. 


In ARIS, the recombination dependences on electron recoil equivalent energy  (E$_{ee}$)\footnote{In case of NRs, E$_{ee}$ = \Leff(E$_{nr}$)$\times$E$_{nr}$.  }  and field (F) are studied with respect to the observable: 


\begin{equation}
{ S1 \over S1_{0} } = { \alpha + R (E_{ee}, F) \over 1 + \alpha},
\label{eqn:zvariable}
\end{equation}

where S1$_0$ is the scintillation response at null field. 

\begin{figure}[t]
\includegraphics[width=\columnwidth]{dokebirks.pdf}
%\caption{Ratio between S1 measured at different drift fields and S1 measured at null field for \ERs\, fit with the Doke-Birks model.}
\caption{Field induced quenching of S1 for \ERs\ at different drift fields, fit with the Doke-Birks model.}
\label{fig:recombination_ER}
\end{figure}

Equation \ref{eqn:zvariable}  is expected to reproduce ARIS data in both ER and NR modes, by accordingly changing the value of $\alpha$, if the   recombination probability $R(E,F)$ is correctly modelled. 
The S1/S1$_0$ ratio extracted from the data is compared with three recombination models:
%We compare S1/S1$_0$ ratio, extracted from the data, with three recombination models:   
Thomas-Imel~\cite{Thomas:1987zz},  Doke-Birks~\cite{Doke:1988kw},  and  PARIS model~\cite{Agnes:2017grb}.  The first is an extension of the Jaffe ``box'' theory \cite{ANDP:ANDP19133471205} and was demonstrated to be accurate in the ``short track'' regime, such as NRs or low energy ERs. The Doke-Birks model is empirical and expected to reproduce data at higher energies. PARIS was tuned on DarkSide-50 data at 200 V/cm only, but was demonstrated to work from $\sim$3~keV up to $\sim$550~keV. 


The Doke-Birks model parametrizes $R$ as the following:

\begin{equation}
R = \frac{A~dE/dx}{1+B~dE/dx} + C,
\end{equation}
where B = A/(1-C) and $dE/dx$ is the energy loss by electrons in LAr. We introduce a  dependence on the electric field, $F$, by defining 

\begin{equation}
C = C'\,e^{-D\times F}. 
\end{equation}




ARIS data in ER mode were simultaneously fit with this electric field-modified version of  Doke-Birks  in the [40,300]~keV$_{ee}$ range, with the results shown in figure \ref{fig:recombination_ER}. The parameters returned by the fit are   A=(2.5$\pm$0.2)$\times$10$^{-3}$ cm/MeV, C'=0.77$\pm$0.01, and D=(3.5$\pm$0.3)$\times$10$^{-3}$ cm/V. With these parameters, the model is able to reproduce ER data with energy from 40 keV at any field. However, while the Doke-Birks   recombination tends to 1  at lower energies, observations from the DarkSide-50 data demonstrate that it should decrease \cite{Agnes:2017grb}. The PARIS model, which was designed to solve this issue, does not require any tuning of the parameters and accurately matches the data, as shown in figure~\ref{fig:recombination_PARIS}.     The difference between Doke-Birks and PARIS models appears for energies below 10~keV$_{ee}$. 

\begin{figure} [!t]
\includegraphics[width=\columnwidth]{paris.pdf}
\caption{Field induced quenching of S1 for \ERs\ at 200 V/cm compared with the PARIS model and the fit of the Doke-Birks model.  The inset shows the same data with the x-axis represented in a log-scale.}
\label{fig:recombination_PARIS}
\end{figure}


NR data, converted in ER equivalent energy by means of the \Leff measured in section \ref{sec:quenching}, are fit with the  Thomas-Imel model, in which the recombination probability is given by  

\begin{equation}
R = 1 - \frac{ln(1 + \xi)}{\xi} ,
\end{equation}

where 
\begin{equation}
\xi = C_{box}\frac{N_i}{F^\beta}.
\end{equation}


$C_{box}$ is a constant depending on  the mean ionization electron velocity $v$ and on the size of the ideal box containing the electron-ion cloud. 



\begin{figure}
\includegraphics[width=\columnwidth]{recombination_NR_field.pdf}
\caption{Field induced quenching of S1 for \NRs\ for different drift fields fit with the Thomas-Imel model. The systematic uncertainties are included in the error bars.  The inset shows the same data with the x-axis represented in a log-scale.}
\label{fig:recombination_NR_field}
\end{figure}






\begin{figure}
\includegraphics[width=\columnwidth]{nr_reco_models.pdf}
\caption{Field induced quenching of S1 for \NRs\ at 200~V/cm compared to model predictions from Thomas-Imel, tuned on the NR data set, and Doke-Birks and PARIS models, tuned on ERs, assuming $\alpha$=1. }
\label{fig:recombination_NR_g4ds}
\end{figure}

Figure \ref{fig:recombination_NR_field} shows the S1/S1$_0$ ratio, at different fields, for NRs, fit with the Thomas-Imel model. The fit returns   $\beta$=1.07$\pm$0.09, in good agreement with the Thomas-Imel prediction of $\beta$=1, and $C_{box}$=18.5$\pm$9.7.  The resulting Thomas-Imel model for NRs is compared with Doke-Birks and PARIS under the paradigm that, with a fixed recombination probability, models should be able to describe both ER and NR data sets by changing the scintillation-to-ionization ratio from $\alpha$=0.21 (ER) to $\alpha$=1 (NR). This paradigm is disproved by the comparison between models and the NR data set at 200 V/cm, shown in figure~\ref{fig:recombination_NR_g4ds}, where Doke-Birks and PARIS predictions are rejected at more than 5$\sigma$.  The Doke-Birks and PARIS models are not recovered in NR mode, even by changing the  $\alpha$ value. 

An overall model requires then two separate recombination probabilities in order to describe both ERs and NRs. In  the range of dark matter searches in LAr ($<$60~keV$_{ee}$),  the tuned Thomas-Imel model was demonstrated to correctly describe scintillation response to NRs, while PARIS is confirmed as a good modeling for ERs, if operating at 200~V/cm. Doke-Birks provides a good description of ERs at different fields, but almost outside the range  of interest ($>$40~keV$_{ee}$) for dark matter searches. 

As a final check, the tuned Thomas-Imel model was used for predicting the number of free ionization electrons

\begin{equation}
N_e =  \mathcal{L}_{eff} \times { E_{dep} \over  W } \frac{1-R(E_{ee},F)}{1+\alpha}
\end{equation}

measured by Joshi et al. \cite{Joshi:2014fna}, as function of the drift field ($F$), for 6.7~keV$_{nr}$ NRs, assuming the \Leff measured in this work. Figure~\ref{fig:joshi} shows excellent agreement, suggesting that, apart from \Leff, no extra-quenching factor affects  S2, which can be essentially modeled as  complementary to S1, under the assumption that the excitation to ionization ratio $\alpha$ is equal to 1 for NRs.  
 
 







\begin{figure}
\includegraphics[width=\columnwidth]{joshi.pdf}
\caption{Comparison of the S2 signal, expressed in number of ionization electrons,  between the \textit{Joshi et al.} data set at 6.7~keV$_{nr}$ and the Thomas-Imel model prediction, as a function of the drift field.}
\label{fig:joshi}
\end{figure}








==> selection.tex <==
% !TEX root = aris_q_paper.tex

\section{Selection criteria}
\label{sec:selection}

%\blue{Editor: Anyssa and Quentin}

In order to understand the different populations  of events in the the data sample, four observables are used:  the two previously defined TOF variables (\TPCtof and  \NDtof), and the TPC  (\FNine) and  ND (\NDpsd) pulse shape variables.  \FNine   is defined as the fraction  of the first 90~ns of the light pulse in the TPC, while  \NDpsd corresponds to the fraction of photoelectrons detected  after 40~ns up to the end of the acquisition gate (7~$\mu$s) in the NDs.  

 

\begin{figure}[t]
	\includegraphics[width=\columnwidth]{selection_tof_tof.pdf}
	\includegraphics[width=\columnwidth]{selection_psd_vs_tof.pdf}
	\includegraphics[width=\columnwidth]{selection_tof_f90.pdf}
	\caption{ \NDtof vs. \TPCtof (top),  \NDpsd vs. \NDtof (center), and \FNine vs. \TPCtof (bottom) for triple coincidences with the A3 detector.  The numbered populations are described within the text. The red lines corresponds to the selection cuts for NRs (D1) and ERs (D2). Yellow lines highlight two classes of NR (D3) and ER backgrounds. }
	\label{fig_selection}
\end{figure}

 
Figure~\ref{fig_selection} shows different combinations of   observables  for triple coincidence events in the A3 ND,   highlighting four different classes of events as well as the selection cuts for NR and ER signals.  The four classes of events described in the subsequent paragraphs are labeled in the figure.

{\bf D1} Large \FNine indicates that these events are mostly NRs, and the values of \mbox{\TPCtof$\sim60$~ns} and \mbox{\NDtof$\sim150$~ns} are in agreement with the  expected TOF from $\sim1.5$~MeV neutrons  traveling 1~m to the TPC    and 2.5~m to the ND.  The    \NDpsd  variable  confirms that these events are neutrons,  with a mean value of  $\sim0.35$ corresponding to the expectation for proton recoil in scintillator from a neutron interaction. 

{\bf D2} The  small \FNine and \NDpsd in combination with TOF values at the few nanosecond scales provide clear indications that these events are beam-generated $\gamma$s interacting in both the TPC and ND.  %The pileup from more than one $\gamma$ produced by the beam pulse and interacting in both detectors is negligible given the measured $\gamma$ rate in the TPC. 

{\bf D3} \FNine classifies   these events as  neutrons, but the  two TOFs are shorter  than for the expected signal from   $\sim$1.5~MeV neutrons. These high energy neutrons are identified as byproducts of fusion-evaporation reactions between the different target materials and the accelerated \Li. 

{\bf D4} The short \NDtof, compatible with   $\gamma$s in the ND, and the long \TPCtof, compatible with neutrons in the TPC,  identify these events as accidental coincidences between a neutron and $\gamma$ correlated with the beam pulse.  

Events in D1 and D2 categories are selected by combining cuts on  \TPCtof, \NDtof, and \NDpsd variables. The selection has been optimized independentely for each ND. As an example, the cuts used for A3 are shown by the red boxes in figure~\ref{fig_selection}. 
The \FNine cut is excluded by the data selection to avoid possible biases in the TPC energy spectra due to the correlation between S1 and \FNine. 

The most significant background to the neutron signal population is from accidental coincidences between a neutron in the TPC and an ambient $\gamma$ in a ND.  A probability density function of the S1 spectrum of this background is produced by selecting events with the same \TPCtof as is used for the D1 signal events, accepting all events in the \NDtof variable that are not coincident with the D1 or D2 region windows.  The background spectrum is normalized to a high energy region of the signal S1 spectrum for NR events, by requiring S1$>500$~pe, and subtracted, as shown in the top plot of figure~\ref{fig_spbkg} for the ND A3.

%These cuts remove background correlated with the beam pulse. Purely accidental background is shown in the continuous bands for \NDtof at the expected \TPCtof for neutrons or $\gamma$s in figure~\ref{fig_selection}.  In the case of the NRs this background is selected by applying the same cut for the \TPCtof used for  category of events D1, and by cutting on the complementary of  D1 and D3 regions in the \NDtof variable. The background spectra in S1 are then statistically subtracted from the signal candidates, as shown in the top plot of figure~\ref{fig_spbkg} for the ND A3. 

In the case of ERs,  $\gamma$s scattering multiple times in the TPC materials is the dominant background, making accidental background subtraction irrelevant. The overall background is   estimated using the \textit{TSpectrum Background} algorithm from \textit{ROOT}~\cite{Brun:1997pa}, as shown in the bottom plot of figure~\ref{fig_spbkg} for  A3. 




			
\begin{figure}
\includegraphics[width=\columnwidth]{selection_spectra_bkg_ch3.pdf}
\includegraphics[width=\columnwidth]{selection_compton_bkg_ch3.pdf}
\caption{Top: NR spectrum in A3 (21.5 keV recoil energy). Bottom: ER spectrum for Compton scattered electrons in  A3. In black is the spectrum after all the selection cuts. The background is represented by the blue histogram.}
\label{fig_spbkg}
\end{figure}
	





==> setup.tex <==
% !TEX root = aris_q_paper.tex

\section{Experimental setup}

\begin{figure}[t]
\includegraphics[width=0.48\columnwidth]{setup_tpc_drawing.pdf}
\includegraphics[width=0.48\columnwidth]{setup_tpc_picture.png}
\caption{Left panel: 3D drawing of the TPC. Right panel: picture of the TPC.}
\label{fig_setup_drawing}
\end{figure}

The ARIS TPC was designed to minimize non-active materials in the direction of the neutron beam to inhibit interaction in passive materials.
The $\sim$0.5 kg  LAr active mass  is housed in a 7.6~cm inner diameter, 1~cm thick Polytetrafluoroethylene (PTFE) sleeve.
The PTFE inner surface includes an embedded Enhanced Specular Reflector (ESR) film for increased light reflection.
The PTFE sleeve supports a set of  2.5~mm thick copper rings connected by resistors in series to maintain a uniform electric field throughout the active argon volume as depicted in figure~\ref{fig_setup_drawing}.  The TPC is held in a double-walled stainless steel dewar.  Evaporated argon is continuously purified with a getter and re-condensed by means of a custom cold head.

The electric field is created by two fused silica windows %which are coated with indium tin oxide (ITO) and 
placed at the end-caps of the cylindrical volume.  The fused silica windows are coated with indium tin oxide (ITO) which is a transparent conductor. 
A hexagonal stainless steel grid is placed %\cmt{9.652 mm} 
1~cm below the anode to enable the creation of an extraction field for a potential S2 signal.  For the measurements presented in this paper, the TPC was operated in single phase without a gas pocket.  The anode is held at ground while the voltages on the extraction grid and cathode are tuned to create a uniform drift field across the entire liquid volume.  The electric field uniformity was confirmed with COMSOL \cite{COMSOL:4.4} simulations, with deviations smaller than 1\% for all drift fields.  
Operation of the TPC in single phase maximizes statistics for the S1 signal, the focus of this work, while limiting pile-up events.


The scintillation photons are wavelength shifted from the ultraviolet to visible range by the tetraphenyl butadine (TPB) compound, which has been evaporated onto all surfaces facing the active volume.  Wavelength shifted photons are observed by one 3-inch R11065 photomultiplier tube (PMT) below the cathode and seven 1-inch R8520 PMTs above the anode.  An optical fiber connected to a LED, powered by a pulse generator, is used to calibrate the single photoelectron response of the PMTs. 

The TPC is mounted with its center 1.00~m away from the LICORNE neutron production target, a hydrogen gas cell which is exposed to a \Li beam that can be accelerated to different energies.
For the measurements presented in this paper the \Li energy was set at 14.63~MeV.  
The gas cell and the beam pipe are separated by a thin tantalum foil where \Li nuclei lose some of their energy. The determination of the \Li energy after the tantalum foil and the parameters of the neutron beam are described in the next section. The \Li beam provides 1.5~ns wide pulses every 400~ns with a current between 20 and 40 nA.  The neutrons reaching the TPC are of the order of 10$^4$~Hz. 

The eight neutron detectors (NDs) surrounding the TPC have active volumes of NE213 liquid scintillator, with a diameter of 20~cm  and an height of 5~cm~\cite{LAURENT1993517}.  The pulse shape of the signal from the liquid scintillator can be used to discriminate between neutrons and $\gamma$s.  The NDs are located at distances from the TPC ranging from 1.3 to 2.5~m, oriented at angles between 25.5 and 133.1 degrees (see table~\ref{tab_NRenergies}). The ND positions were precisely measured before the data taking with a survey method yielding an accuracy of 2-3~mm, depending on the ND.  An inspection after the data taking identified a mismatch between the recorded position of A2 and its position during data taking, which is reflected in a larger systematic uncertainty for measurements using that data point, described in further detail in section~\ref{sec:quenching}.

	\begin{table}
	\centering
	\begin{tabular}{c |  c | c | c}
		\hline
		\hline
					&	 Scattering	&	Mean NR			&	Mean ER \\
					&	Angle [deg]	&	Energy [keV]		&	Energy [keV]\\
       		\hline 
			A0		&	25.5			&	7.1	                 & 42.0                  \\
			A1		&	35.8			&	13.7		         & 75.9                  \\
			A2		&	41.2			&	17.8		         & 85.8                  \\
			A3		&	45.7			&	21.7		         & 110.3                  \\
			A4		&	64.2			&	40.5		         & 174.5                 \\
			A5		&	85.5			&	65.4		         & 232.0 		   \\
			A6		&	113.2		&	98.1		        & 282.7			\\
			A7		&	133.1		&	117.8		& 304.9              \\
		\hline
		\hline
	\end{tabular}
	\caption{Scattering angles, NR mean energies for neutrons from the \Lipn reaction, and ER mean energies from Compton scattered $\gamma$s emitted by \Lim de-excitation, are shown. The scattering angle is defined with respect to the center of the NDs active surface while the mean energies are determined with Monte Carlo simulations.}
	\label{tab_NRenergies}
	\end{table}
 
Data taking occurred during a 12 day period in October 2016 with various electric fields in the TPC, ranging from 0 to 500~V/cm. Data were taken in two modes: double coincidence mode  between the beam pulse and a TPC trigger, and a triple coincidence mode which included also coincidence with at least one of the NDs. The TPC trigger condition requires at least  two PMTs to fire within 100 ns and a measurement of the TPC trigger efficiency will be described in section~\ref{sec_calibration}.  The triple coincidence data set provides nuclear and electronic recoils of defined energies. %, as quoted in table~\ref{tab_NRenergies}. 
The double coincidence data, which provides continuous spectra, are used for an investigation of the LAr scintillation time response, which will be presented in a future publication. 

When a trigger occurs signals from the  TPC PMTs and from A0--A7 are digitized by two CAEN V1720 boards at a 250~MHz frequency. The time of the beam pulses is also digitized at a 250~MHz frequency by a CAEN V1731 board.  The board timestamps are synchronized by an external clock to allow for time-of-flight measurements. 

For each coincidence, the TPC PMT waveforms, the ND waveforms, and the signal from the beam pulse are recorded.  The acquisition window was 10~$\mu$s for the TPC PMTs and 7~$\mu$s for each ND. The signals are analyzed by a reconstruction software based on the \textit{art} framework \cite{Green:2012gv} to extract observables from the recorded waveforms.  First, fluctuations and drift of the baseline are tracked and subtracted from the raw signal waveforms.  Next, waveforms from each PMT in the TPC are corrected for their single photoelectron response and summed together.  A pulse finder algorithm is applied to each summed waveform to identify the magnitude and start time of TPC and ND pulses.  Finally, the reconstructed waveform and pulse information are used to extract the \SOne amplitude, pulse shape discrimination parameters for both the TPC and NDs, and time-of-flight (TOF) parameters.  %The final observables are used for the data selection and analyses reported in the subsequent sections of this work.


A Geant4-based Monte Carlo simulation of the experimental setup has been developed which includes the materials, size, and relative placement of the TPC, PMTs, dewar, and A0--A7 detectors as described above.  The beam kinematics is also included as described in section~\ref{sec:BeamKinematics}. This simulation provides a spectrum of nuclear and electronic recoil energies from coincidences between the TPC and A0--A7 detectors, with mean values listed in table~\ref{tab_NRenergies}.


%In order to maximize the statistics, the gas pocket was suppressed during the entire data taking. The drift time, in fact, requires an acquisition window up to hundreds of microseconds, depending on the electric field, exposing the TPC to a large pile-up   with accidental background. The lack of  the S2 signal, although preserving the electric field, allows to reduce the acquisition window to 10~$\mu$s and hence the background. At the same time it does not prevent to infer the amplitude of the ionization component thanks to the accurate determination of the recoil energy.  -- this part can be taken out as it is described in a previous paragraph.

